APPO: Attention-guided Perception Policy Optimization for Video Reasoning

Complex video reasoning, actually, relies excessively on fine-grained perception rather than on expert (e.g., Ph.D, Science)-level reasoning. Through extensive empirical observation, we have recognized the critical impact of perception. In particular, when perception ability is almost fixed, enhancing reasoning from Qwen3-8B to OpenAI-o3 yields only 0.7% performance improvement. Conversely, even minimal change in perception model scale (from 7B to 32B) boosts performance by 1.4%, indicating enhancing perception, rather than reasoning, is more critical to improve performance. Therefore, exploring how to enhance perception ability through reasoning without the need for expensive fine-grained annotation information is worthwhile. To achieve this goal, we specially propose APPO, the Attention-guided Perception Policy Optimization algorithm that leverages token-level dense rewards to improve model's fine-grained perception. The core idea behind APPO is to optimize those tokens from different responses that primarily focus on the same crucial video frame (called intra-group perception tokens). Experimental results on diverse video benchmarks and models with different scales (3/7B) demonstrate APPO consistently outperforms GRPO and DAPO (0.5%~4%). We hope our work provides a promising approach to effectively enhance model's perception abilities through reasoning in a low-cost manner, serving diverse scenarios and demands.

==> sec/0_abstract.tex <==
\begin{abstract}
Complex video reasoning, actually, relies excessively on fine-grained perception rather than on expert (\emph{e.g.}, Ph.D, Science)-level reasoning.
Through extensive empirical observation, we have recognized the critical impact of perception.
In particular, when perception ability is almost fixed, enhancing reasoning from Qwen3-8B to OpenAI-o3 yields only $0.7\%$ performance improvement. Conversely, even minimal change in perception model scale (from 7B to 32B) boosts performance by $1.4\%$, indicating enhancing perception, rather than reasoning, is more critical to improve performance.
Therefore, exploring how to enhance perception ability through reasoning without the need for expensive fine-grained annotation information is worthwhile.
To achieve this goal, we specially propose \textbf{APPO}, the \textbf{A}ttention-guided \textbf{P}erception \textbf{P}olicy \textbf{O}ptimization algorithm that leverages token-level dense rewards to improve model's fine-grained perception.
The core idea behind APPO is to optimize those tokens from different responses that primarily focus on the same crucial video frame (called intra-group perception tokens).
Experimental results on diverse video benchmarks and models with different scales ($3$/$7$B) demonstrate APPO consistently outperforms GRPO and DAPO ($0.5\%\sim4\%$). 
We hope our work provides a promising approach to effectively enhance model's perception abilities through reasoning in a low-cost manner, serving diverse scenarios and demands.
\end{abstract}





==> tabs/ab_alpha.tex <==



\begin{table}[t]\small
\centering
\caption{Ablation results for $\alpha$ on SEED-Bench-R1 Benchmark.}
\vspace{-1em}
\addtolength\tabcolsep{-2.4pt}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\alpha & L1 (In-Dist.) & L2 (OOD) & L3 (OOD) \\
\midrule
% \rowcolor{gray!15}\multicolumn{4}{c}{\textbf{Qwen2.5-VL-3B}} \\
% \alpha=1.2 &  & &  \\
% \alpha=1.4 & &  &  \\
% \alpha=1.7 &      &      &      \\
% \alpha=2.0 &  &  &  \\
% \midrule

% \rowcolor{gray!15}\multicolumn{4}{c}{\textbf{Qwen2.5-VL-7B}} \\
1.2 & 48.5 & 48.9 & 46.9 \\
1.4 & 48.1 & 50.2 & 45.7 \\
1.7 & 49.1 & 50.7 & 48.4 \\
2.0 & 48.7 & 49.2 & 46.5 \\


\bottomrule
\end{tabular}
}
% \vspace{-2mm}
% \vspace{-2mm}
\label{tab:alpha} 
\end{table}









==> tabs/ab_alpha_K1.tex <==



\begin{table}[t]\small
\centering
\caption{Ablation results for $\alpha$ on SEED-Bench-R1 Benchmark.}
\vspace{-1em}
\addtolength\tabcolsep{-2.4pt}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|c|ccc}
\toprule
\multicolumn{1}{c|}{Parameter} & L1 (In-Dist.) & L2 (OOD) & L3 (OOD) \\
\midrule
% \rowcolor{gray!15}\multicolumn{4}{c}{\textbf{Qwen2.5-VL-3B}} \\
% \alpha=1.2 &  & &  \\
% \alpha=1.4 & &  &  \\
% \alpha=1.7 &      &      &      \\
% \alpha=2.0 &  &  &  \\
% \midrule

% \rowcolor{gray!15}\multicolumn{4}{c}{\textbf{Qwen2.5-VL-7B}} \\
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{\alpha}}} & 1.2 & 48.5 & 48.9 & 46.9 \\
% \multicolumn{1}{c|}{} & 1.4 & 48.1 & 50.2 & 45.7 \\
% \multicolumn{1}{c|}{} & 1.7 & 49.1 & 50.7 & 48.4 \\
% \multicolumn{1}{c|}{} & 2.0 & 48.7 & 49.2 & 46.5 \\

$\alpha=1.2$ & 48.5 & 48.9 & 46.9 \\
$\alpha=1.4$ & 48.1 & 50.2 & 45.7 \\
$\alpha=1.7$ & 49.1 & 50.7 & 48.4 \\
$\alpha=2.0$ & 48.7 & 49.2 & 46.5 \\

\midrule

$K_1=8$ & 49.4 & 49.7 & 47.4 \\
$K_1=15$ & 49.1 & 50.7 & 48.4 \\
$K_1=30$ & 49.6 & 51.2 & 48.8 \\

% \midrule

% $K_2=1$ & 49.4 & 49.7 & 47.4 \\
% $K_2=3$ & 49.1 & 50.7 & 48.4 \\
% $K_2=5$ & 49.3 & 51.2 & 48.8 \\
% $K_2=8$ & 49.3 & 51.2 & 48.8 \\


% \midrule

% $K_3=64$ & 49.4 & 49.7 & 47.4 \\
% $K_3=128$ & 49.1 & 50.7 & 48.4 \\
% $K_3=256$ & 49.3 & 51.2 & 48.8 \\
% $K_3=512$ & 49.3 & 51.2 & 48.8 \\


\bottomrule
\end{tabular}
}
% \vspace{-2mm}
% \vspace{-2mm}
\label{tab:alpha} 
\end{table}












==> tabs/ab_k2_k3.tex <==



\begin{table}[t]\small
\centering
\caption{Ablation results for $\alpha$ on SEED-Bench-R1 Benchmark.}
\vspace{-1em}
\addtolength\tabcolsep{-2.4pt}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|c|ccc}
\toprule
\multicolumn{1}{c|}{Parameter} & L1 (In-Dist.) & L2 (OOD) & L3 (OOD) \\
\midrule
% \rowcolor{gray!15}\multicolumn{4}{c}{\textbf{Qwen2.5-VL-3B}} \\
% \alpha=1.2 &  & &  \\
% \alpha=1.4 & &  &  \\
% \alpha=1.7 &      &      &      \\
% \alpha=2.0 &  &  &  \\
% \midrule

% \rowcolor{gray!15}\multicolumn{4}{c}{\textbf{Qwen2.5-VL-7B}} \\
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{\alpha}}} & 1.2 & 48.5 & 48.9 & 46.9 \\
% \multicolumn{1}{c|}{} & 1.4 & 48.1 & 50.2 & 45.7 \\
% \multicolumn{1}{c|}{} & 1.7 & 49.1 & 50.7 & 48.4 \\
% \multicolumn{1}{c|}{} & 2.0 & 48.7 & 49.2 & 46.5 \\

$K_2=1$ & 48.0 & 49.8 & 47.3 \\
$K_2=3$ & 49.9 & 50.9 & 49.7 \\
$K_2=5$ & 49.1 & 50.7 & 48.4 \\
$K_2=8$ & 48.1 & 51.0 & 45.6 \\

\midrule

$K_3=64$ & 48.1 & 51.6 & 48.1 \\
$K_3=128$ & 48.7 & 50.6 & 49.5 \\
$K_3=256$ & 48.3 & 50.9 & 48.7 \\
$K_3=512$ & 49.1 & 50.7 & 48.4 \\


\bottomrule
\end{tabular}
}
% \vspace{-2mm}
% \vspace{-2mm}
\label{tab:alpha} 
\end{table}














==> tabs/ab_sampling.tex <==



\begin{table}[t]\small
\centering
\caption{Ablation results for dynamic sampling on SEED-Bench-R1 Benchmark.}
\vspace{-1em}
\addtolength\tabcolsep{-2.4pt}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
Sampling & L1 (In-Dist.) & L2 (OOD) & L3 (OOD) \\
\midrule
% \rowcolor{gray!15}\multicolumn{4}{c}{\textbf{Qwen2.5-VL-3B}} \\
% \alpha=1.2 &  & &  \\
% \alpha=1.4 & &  &  \\
% \alpha=1.7 &      &      &      \\
% \alpha=2.0 &  &  &  \\
% \midrule

% \rowcolor{gray!15}\multicolumn{4}{c}{\textbf{Qwen2.5-VL-7B}} \\
sampling-3b &  & &  \\
3b & 37.5 & 39.1 & 35.0 \\
sampling-7b & 49.7 & 51.1 & 49.5 \\
7b & 50.5 & 51.3 & 49.3 \\


\bottomrule
\end{tabular}
}
% \vspace{-2mm}
% \vspace{-2mm}
\label{tab:sampling} 
\end{table}













